Decentralize and Randomize: Faster Algorithm for Wasserstein Barycenters

We study the decentralized distributed computation of discrete approximations for the regularized Wasserstein barycenter of a finite set of continuous probability measures distributedly stored over a network. We assume there is a network of agents/machines/computers, and each agent holds a private continuous probability measure and seeks to compute the barycenter of all the measures in the network by getting samples from its local measure and exchanging information with its neighbors. Motivated by this problem, we develop, and analyze, a novel accelerated primal-dual stochastic gradient method for general stochastic convex optimization problems with linear equality constraints. Then, we apply this method to the decentralized distributed optimization setting to obtain a new algorithm for the distributed semi-discrete regularized Wasserstein barycenter problem. Moreover, we show explicit non-asymptotic complexity for the proposed algorithm.

==> von_mises.tex <==
\begin{figure}[htbp!]
	\centering
	
%	\subfigure{\begin{tikzpicture}
%		\begin{axis}[
%		ticklabel style = {font=\tiny},
%		width=3.8cm,height=4cm,scale=0.99,
%		x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\small},
%%		y label style={at={(axis description cs:0.25,.5)},anchor=south},
%		xlabel={$x, N=1$},
%%		ymode = log,
%%		xmode = log,
%		ymin = 0, ymax=0.1,
%		xmin = -5, xmax=5, 
%		cycle list name=color list,
%		every axis plot/.append style={line width=1pt},
%		ytick={0,0.1},
%		yticklabels={$0$,$0.1$}],
%		legend pos=south west;
%		\addplot     	table [x index=40,y index=0]{ex7.dat};
%		\addplot     	table [x index=40,y index=1]{ex7.dat};
%		\addplot      	table [x index=40,y index=2]{ex7.dat};
%		\addplot      	table [x index=40,y index=3]{ex7.dat};
%		\addplot     	table [x index=40,y index=4]{ex7.dat};
%		\addplot     	table [x index=40,y index=5]{ex7.dat};
%		\addplot      	table [x index=40,y index=6]{ex7.dat};
%		\addplot      	table [x index=40,y index=7]{ex7.dat};
%		\addplot      	table [x index=40,y index=8]{ex7.dat};
%		\addplot      	table [x index=40,y index=9]{ex7.dat};
%		\end{axis}
%		\end{tikzpicture}
%	}
%	\subfigure{\begin{tikzpicture}
%	\begin{axis}[
%	ticklabel style = {font=\tiny},
%	width=3.8cm,height=4cm,scale=0.99,
%	x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\small},
%	%		y label style={at={(axis description cs:0.25,.5)},anchor=south},
%	xlabel={$x, N=100$},
%	%		ymode = log,
%	%		xmode = log,
%	ymin = 0, ymax=0.1,
%	xmin = -5, xmax=5, 
%	cycle list name=color list,
%	every axis plot/.append style={line width=1pt},
%	ytick={0,0.1},
%	yticklabels={$0$,$0.1$}],
%	legend pos=south west;
%	\addplot     	table [x index=40,y index=10]{ex7.dat};
%	\addplot     	table [x index=40,y index=11]{ex7.dat};
%	\addplot      	table [x index=40,y index=12]{ex7.dat};
%	\addplot      	table [x index=40,y index=13]{ex7.dat};
%	\addplot     	table [x index=40,y index=14]{ex7.dat};
%	\addplot     	table [x index=40,y index=15]{ex7.dat};
%	\addplot      	table [x index=40,y index=16]{ex7.dat};
%	\addplot      	table [x index=40,y index=17]{ex7.dat};
%	\addplot      	table [x index=40,y index=18]{ex7.dat};
%	\addplot      	table [x index=40,y index=19]{ex7.dat};
%	\end{axis}
%	\end{tikzpicture}
%}
%	\subfigure{\begin{tikzpicture}
%	\begin{axis}[
%	ticklabel style = {font=\tiny},
%	width=3.8cm,height=4cm,scale=0.99,
%	x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\small},
%	%		y label style={at={(axis description cs:0.25,.5)},anchor=south},
%	xlabel={$x, N=200$},
%	%		ymode = log,
%	%		xmode = log,
%	ymin = 0, ymax=0.1,
%	xmin = -5, xmax=5, 
%	cycle list name=color list,
%	every axis plot/.append style={line width=1pt},
%	ytick={0,0.1},
%	yticklabels={$0$,$0.1$}],
%	legend pos=south west;
%	\addplot     	table [x index=40,y index=20]{ex7.dat};
%	\addplot     	table [x index=40,y index=21]{ex7.dat};
%	\addplot      	table [x index=40,y index=22]{ex7.dat};
%	\addplot      	table [x index=40,y index=23]{ex7.dat};
%	\addplot     	table [x index=40,y index=24]{ex7.dat};
%	\addplot     	table [x index=40,y index=25]{ex7.dat};
%	\addplot      	table [x index=40,y index=26]{ex7.dat};
%	\addplot      	table [x index=40,y index=27]{ex7.dat};
%	\addplot      	table [x index=40,y index=28]{ex7.dat};
%	\addplot      	table [x index=40,y index=29]{ex7.dat};
%	\end{axis}
%	\end{tikzpicture}
%}
%	\subfigure{\begin{tikzpicture}
%	\begin{axis}[
%	ticklabel style = {font=\tiny},
%	width=3.8cm,height=4cm,scale=0.99,
%	x label style={at={(axis description cs:0.5,-0.1)},anchor=north,font=\small},
%	%		y label style={at={(axis description cs:0.25,.5)},anchor=south},
%	xlabel={$x, N=500$},
%	%		ymode = log,
%	%		xmode = log,
%	ymin = 0, ymax=0.1,
%	xmin = -5, xmax=5, 
%	cycle list name=color list,
%	every axis plot/.append style={line width=1pt},
%	ytick={0,0.1},
%	yticklabels={$0$,$0.1$}],
%	legend pos=south west;
%	\addplot     	table [x index=40,y index=30]{ex7.dat};
%	\addplot     	table [x index=40,y index=31]{ex7.dat};
%	\addplot      	table [x index=40,y index=32]{ex7.dat};
%	\addplot      	table [x index=40,y index=33]{ex7.dat};
%	\addplot     	table [x index=40,y index=34]{ex7.dat};
%	\addplot     	table [x index=40,y index=35]{ex7.dat};
%	\addplot      	table [x index=40,y index=36]{ex7.dat};
%	\addplot      	table [x index=40,y index=37]{ex7.dat};
%	\addplot      	table [x index=40,y index=38]{ex7.dat};
%	\addplot      	table [x index=40,y index=39]{ex7.dat};
%	\end{axis}
%	\end{tikzpicture}
%}
	\caption{Local barycenter generated by the Algorithm~\ref{alg:main} for a set of $10$ agents over an Erd\H{o}s-R\'enyi random graph at different iteration numbers. Each agent can access private realizations from a random variable with a von Mises distribution.}
	\label{fig:von_mises}
\end{figure} 
